GeoDiffuser: Geometry-Based Image Editing with Diffusion Models

The success of image generative models has enabled us to build methods that can edit images based on text or other user input. However, these methods are bespoke, imprecise, require additional information, or are limited to only 2D image edits. We present GeoDiffuser, a zero-shot optimization-based method that unifies common 2D and 3D image-based object editing capabilities into a single method. Our key insight is to view image editing operations as geometric transformations. We show that these transformations can be directly incorporated into the attention layers in diffusion models to implicitly perform editing operations. Our training-free optimization method uses an objective function that seeks to preserve object style but generate plausible images, for instance with accurate lighting and shadows. It also inpaints disoccluded parts of the image where the object was originally located. Given a natural image and user input, we segment the foreground object using SAM and estimate a corresponding transform which is used by our optimization approach for editing. GeoDiffuser can perform common 2D and 3D edits like object translation, 3D rotation, and removal. We present quantitative results, including a perceptual study, that shows how our approach is better than existing methods. Visit https://ivl.cs.brown.edu/research/geodiffuser.html for more information.

==> images/figures_and_tables_tex/removal_loss.tex <==
\begin{figure}[!htb]
  \centering
  \includegraphics[width=\textwidth,height=0.3\textwidth]{example-image-b}
  \caption{\coolname Removal Loss Illustrated}
  \label{fig:removal}
\end{figure}

==> text/09_rebuttal.tex <==
We thank the reviewers for their valuable feedback \& positive comments such as \coolname ``\textbf{provides attractive quantitative \& qualitative results}" (\Rfive) \& ``shows \textbf{consistent improvement over warp loss} \& competitive scores across other metrics" (\Rtwo) in various different scenarios (\Rthree).
We are glad that \Rtwo{} finds our method a ``\textbf{simple optimization-based scheme}" but shows ``\textbf{consistent improvement...and competitive scores...}''---we strongly believe this simplicity is a feature, not a bug.
% (\Rtwo) that transforms ``\textbf{attention with explicit transformation matrix for 3D editing}" (\Rfive). 
% Reviewers agree that our method % Additionally, GeoDiffuser is the \textbf{first method that subsumes an explicit 3D transformation matrix in T2I diffusion models to edit images without any training}.
In this rebuttal, we address reviewer questions and concrete improvements (highlighted in \cbEdit{bluish-green} in the manuscript \& \sm) that will make our final paper stronger.
% \srinath{Say something positive: we are confident that with the clarification \& changes (highlighted in red in the manuscript), it will address all reviewer concerns.}
% \srinath{use supp. instead of SM, it's more standard}
We use short forms \underline{\manu} for manuscript \& \underline{\sm} for supplement. 
% \rahul{Maybe LP for line in paper \& LS for line in supp. is a better shortform}

% \rahul{I will need to update all lines \& sections once we are done with all edits}


\parahead{\underline{Novelty (\Rtwo{}) \& Motivation for \coolname (\Rthree)}} \coolname is the \textbf{first method that bakes explicit 3D transformation within attention layers of T2I models to perform 3D consistent geometric edits with the bonus of being simple}. 
Prior drag-style methods such as DragonDiffusion, FreeDrag, \& more move objects, but their edits are \textbf{not geometry consistent even when the drags are obtained using 3D transformations \& depth maps} (see analysis in section \textit{Evaluation \& Baselines} of \sm). 
% This occurs because these methods locally average nearby drags during optimization resulting in high \textbf{MD} \& \textbf{Warp} errors (Tab \todo{} \& SM. \todo).
Diffusion Handles subsumes 3D transformation to edit \textbf{but it is limited to depth-conditioned models, requires in-distribution depth maps, offloads inpainting dis-occlusions to LaMa \& fails to preserve the appearance of the scene}.
Text-based editing methods such as InstructPix2Pix, Prompt-to-Prompt \textbf{do not allow fine-grained control to transform the geometry of the object} disabling users from rotating \& translating objects within images.
Our simple method of transforming attention beats prior works quantitatively (\manu Tab. 1) \& qualitatively (\manu Fig. 4 \& \sm Fig. 9-11) to perform geometric edits. 
% We display visual 3D editing comparison in the \manu Fig. 4 \& move all other qualitative results to \sm.


\parahead{\underline{Comparison to Diffusion Self-Guidance (DSG) (\Rthree)}}
We include qualitative (\manu Fig. 4) \& quantitative comparison (\manu Tab. 1) to Diffusion SG. 
Refer \sm sec. C.5 for implementation, timing, \& performance analysis. 

\parahead{\underline{Loss Ablations (\Rtwo{}, \Rfive{})}}
We ablate loss functions \& include a discussion for it (see \textit{Ablation} section in \manu).

\parahead{\underline{Gains of Geometric Attention Sharing (\Rtwo{})}} We moved the ablation on performance gains of geometric attention from \sm Tab. 1 to \manu Tab. 2. 
Enabling geometric attention sharing for longer time steps reduces \textbf{MD} \& \textbf{Warp} errors displaying its efficacy in editing. 
% \rahul{}

\parahead{\underline{Inference Runtime (\Rthree{}, \Rfive{}) \& Size of Study (\Rfive)}} 
\coolname performs removal in 30 seconds \& 3D edits in 45 seconds (see \manu L:621). 
This runtime includes inversion, optimization, \& generation with 50 diffusion steps. 
Our work is faster than all baselines except DragonDiffusion that does not perform geometry projection \& benefits from memory bank that can speed our future works.
Our study includes 53 participants (\manu L:729).
% \srinath{say: as already mentioned in the manu.~line xx, our study included...}. 
% \rahul{They write that the number of participants are not clearly visible as it was in our \sm earlier. So I think its fine to just mention that we moved it in the main paper.}
% We already included these in Round 1 \sm L:417 \& in Round 1 \sm L:597 respectively.
% We moved inference time \& user study to \manu L:612 \& L:718 respectively.
% in Round 2 for better readability. 
% \rahul{There should be a better \& concise way to write this}



% Concurrent works such as InstaDrag \& MagicFixup perform edits by training over video data for drag-edits. 
% Two advantages of these works include: 1) the inpainting for in/near-distribution images will be accurate \& 2) faster inference. 
% However, these methods \& in-general video diffusion models face these disadvantages: 1) moving the subject also introduces background movement as video datasets do not distinguish between subject \& background motion, 2) they do not bake geometry within their architecture leading to edits that do not respect geometry, 3) these models are trained with optical flow within a bounded range \& often lose object details \& identity when the motion is beyond this range, \& lastly 4) these models do not explore having inference time optimization disabling the user to control different aspects of the edit by merely changing loss weights. 
% We believe that the geometry attention sharing \& loss functions from \coolname can help improve these models to ensure geometry consistent edits \& generation in future works.
% \rahul{Maybe we can just mention that we added the discussion somewhere in the paper to save space}

% \rahul{The below can be aggregated to one big point?}
\parahead{\underline{Why Direct Inversion? (\Rfive)}} Direct Inversion initializes the reference latents with the inversion trajectory for perfect image reconstruction without the need for optimizing embeddings (null-text) \& weights (LoRA) (see \manu L:430).
% We include this reason in L:422 of the \manu
% \rahul{Do I need to explain this here or just mention it in paper \& reference it here?}

\parahead{\underline{Transform $\mathbf{\mathcal{F}}$ Applied to Query, Geometry Sharing} \underline{Cross Attention (\Rfive)}} 
Applying transformation to the reference query \& then taking dot product with the reference key embeddings provides us with correspondences between the two. 
This edited attention map attends to the reference value embeddings \& ensures that the transform only changes the geometry \& preserves the appearance of the object (see \manu L:529).
We use edit key embeddings within cross-attention layer to enable gradients to the null-text embeddings for optimization (see \manu L:534).

\parahead{\underline{Editing Without Optimization? (\Rtwo, \Rfive)}} Editing without optimization leads to object duplication as our geometric attention sharing mechanism only moves the object but does not remove it from its original location (see \sm Fig. 7 \& \manu L:558). 
Prior works such as Prompt-to-Prompt allow replacing objects/changing appearance without optimization by replacing the cross attention maps corresponding to the text.
However, this does not remove objects \& merely replaces them as the self-attention maps are not changed. 
Optimization enables editing the self-attention map to remove objects instead of change in appearance.
% This is why our work along with prior geometry editing works optimize to inpaint disocclusions \& move the object.
% To remove an object, we need to edit the self-attention map as well to realistically inpaint the dis-occlusions.
% Optimization inpaints the dis-occlusions resulting from the edit.


\parahead{\underline{Pseudo-code (\Rfive{})}} We already included pseudo-code for editing, attention-sharing mechanism, \& removal loss in the \sm of Round 1 Algorithm 1, 2, \& 3 for readability.

% \parahead{\underline{Discussion on In-painting such as Prompt to Prompt (\Rtwo)}} 

% Prompt-to-Prompt allows replacing objects/changing appearance without optimization. 
% This is possible by swapping cross attention layers \& keeping the self-attention as is, however, to remove objects we need to manipulate the self-attention such that it can complete the background. 
% This is why we need to optimize in-order to fill the self-attention for object removal.
% \rahul{We can possibly merge this to before}

\parahead{\underline{Discussion of Concurrent Works MagicFixup \&} \underline{InstaDrag (\Rthree)}} 
Thank you for the suggestion \Rthree{}! We added a discussion in \manu L:247 \& \sm sec. M.

\parahead{\underline{Editing Humans \& Complicated Shapes (\Rthree{})}}
We show edits on humans \& complex shapes (\sm Fig. 14 \& website).
Our edits are limited by the capabilities of the base model \& can improve once trained on such datasets. 
% A generative m
% Our general editing method can be applied to edit humans \& complicated shapes for diffusion models trained on such data.
% \rahul{Try some examples}

\parahead{\underline{Limitation - Rotation Edits (\Rfive{})}} Rotation beyond 45-60$^\circ$ is a very difficult \& requires synthesizing novel views of the object (see \manu L:855).
To our knowledge, there are no editing methods that can do this consistently.
% We share this limitation with prior editing works \& already mention it in \manu L:809.
We include visual 3D edits with a website in \sm


\parahead{\underline{Dataset Size (\Rfive{})}} 
Unlike prior works, we perform all our evaluations on \textbf{real} images from Adobe Stock.
Real images \textbf{incorporate challenging illumination scenarios \& out of distribution images} to evaluate the efficacy of editing works.
% by incorporating real-world illuminations \& out of distribution images.
% \srinath{Say why the use of real images is important \& different from other work.}
% These images are selected to incorporate various categories \& challenging lighting effects such as shadows \& reflections to measure editing performance.
% Our method allows editing in-the-wild as it is purely based on optimization.
% As our method is purely optimization-based enabling it to be applied to any image in the wild. 
Unlike minor drags explored in prior works, proposing large edits for real-images is time-intensive \& \textbf{can not be randomized as these edits need to be scene consistent/plausible.}
% Since our method is training-free, the evaluation dataset belongs to the test set \& scales up with in-the-wild images.
Similar to our method, prior accepted works such as Diffusion Handles, Prompt-to-Prompt, Diffuson Self Guidance perform evaluation on datasets of the same (or even smaller) scale as these methods do not require training \& edit in-the-wild images.

We thank all the reviewers for their suggestions, comments, \& references that will improve our work.
% We are confident that the concrete improvements mentioned above will make our final manuscript stronger.
% \srinath{MOve this to intro.}
